Investigating Lexical Replacements for Arabic-English Code-Switched Data Augmentation

Data sparsity is a main problem hindering the development of code-switching (CS) NLP systems. In this paper, we investigate data augmentation techniques for synthesizing dialectal Arabic-English CS text. We perform lexical replacements using word-aligned parallel corpora where CS points are either randomly chosen or learnt using a sequence-to-sequence model. We compare these approaches against dictionary-based replacements. We assess the quality of the generated sentences through human evaluation and evaluate the effectiveness of data augmentation on machine translation (MT), automatic speech recognition (ASR), and speech translation (ST) tasks. Results show that using a predictive model results in more natural CS sentences compared to the random approach, as reported in human judgements. In the downstream tasks, despite the random approach generating more data, both approaches perform equally (outperforming dictionary-based replacements). Overall, data augmentation achieves 34% improvement in perplexity, 5.2% relative improvement on WER for ASR task, +4.0-5.1 BLEU points on MT task, and +2.1-2.2 BLEU points on ST over a baseline trained on available data without augmentation.

==> sections/arzen.tex <==
\section{ArzEn Parallel Corpus}
\label{sec:arzenMT}
%CS occurs most commonly in speech, which makes the process of collecting such CS data challenging and restricted. 
We present our work on collecting the first parallel corpus for CS Egyptian Arabic and English.\footnote{The corpus and guidelines will be made available.} We collect our corpus by translating ArzEn speech corpus \newcite{HVA20}\footnote{We thank \cite{HVA20} for allowing us early access to the corpus, which we understand will be released soon.} which consists of informal interviews discussing broad topics, such as education and life experiences. The corpus consists of $6,290$ sentences having $99,340$ words. In Table~\ref{table:arzen}, we provide an overview of ArzEn corpus.

\begin{table}[t]
\centering
%\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l r}
      \hline
      \multicolumn{2}{c}{\textbf{ArzEn Speech Corpus}} \\\hline
      Duration&12h\\
      \#Speakers&40\\
      \# Sentences&6,290\\
      \# Tokens&102,332\\
      \% CS sentences&63.2\%\\
      \% English words in CM sentences&18.7\%\\
      \% Sentences with morphological CS&28.7\%\\
      \# Morphological CS Words & 2,684\\\hline
      %\multicolumn{2}{|c|}{\textbf{Inter-sentential CS}} \\\hline
      %\% Monolingual Arabic Sentences&33.1\%\\\hline
      %\% Monolingual English Sentences&3.7\%\\\hline
      %\multicolumn{2}{|c|}{\textbf{Intra-sentential CS}} \\\hline
      %\% CS Sentences&63.2\%\\\hline
      %\% Arabic Tokens&84.9\%\\\hline
      %\% English Tokens&15.1\%\\\hline
\end{tabular}
%}
\caption{ArzEn corpus overview.}
\label{table:arzen}
\end{table}

The corpus was translated by professional translators and the test and dev sets were revised by the translators and one of the authors. Our guidelines generally follow the LDC Arabic-to-English Translation Guidelines \cite{LDC13}. We modified the guidelines with regards to CS segments. % such that source text English words are annotated in the target text with a  hashtag prefix to allow for further linguistic analysis (Table~\ref{table:arzen_examples},~example~1). 
In the LDC guidelines, it is recommended that embedded English segments in the source text should be copied to target text without changes or corrections. We allow modifications for better fluency and to handle morphological CS. The translators were also asked to mark the CS segments occurring on the source side in the provided translations using a hashtag prefix to allow for further linguistic analysis. 
Examples are given in Table~\ref{table:arzen_examples}.

\begin{comment}
\begin{table}[t]
\centering
%\resizebox{0.7\columnwidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|l|r|}
      \hline
%      \multicolumn{1}{|c}{\textbf{Category}}&\multicolumn{1}{|c|}{\textbf{Value}}\\
%      \hline
%      \# Sentences & 6,290\\\hline
%      \# Words & 99,340\\\hline
%      \# Tokens&102,332\\\hline
      %\multicolumn{2}{|c|}{\textbf{Inter-sentential CS}} \\\hline
      %\% Monolingual Arabic Sentences&33.1\%\\\hline
      %\% Monolingual English Sentences&3.7\%\\\hline
      \multicolumn{2}{|c|}{\textbf{Intra-sentential CS}} \\\hline
      \% CS Sentences&63.2\%\\\hline
      %\% Arabic Tokens&84.9\%\\\hline
      \% English Tokens&15.1\%\\\hline
      \multicolumn{2}{|c|}{\textbf{Morphological CS}} \\\hline
      %\% Sentences with morphological CS&28.4\%\\\hline
      \% CS sentences with morphological CS&45.0\%\\\hline
      %\% Morphological CS words & 2.7\%\\\hline
      \# Morphological CS Words & 2,684\\\hline
\end{tabular}
%}
\caption{ArzEn Corpus codeswitching (CS) frequency.}
\label{table:arzen}
\end{table}
\end{comment}

\begin{comment}
\begin{table}
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|l|r|}
\hline
\multicolumn{2}{|c|}{\textbf{Example 1}}\\\hline
src&
project code
\<انا كتبت ال>\\
trg&\multicolumn{1}{l|}{I wrote the \#project \#code}\\\hline
\multicolumn{2}{|c|}{\textbf{Example 2}}\\\hline
src&
intership
\<عملت كذا>\\
trg&\multicolumn{1}{l|}{I did several \#internships}\\\hline
\multicolumn{2}{|c|}{\textbf{Example 3}}\\\hline
src&
\<الناس اللى معايا>
overload 
\<كنت ب>\\
trg&\multicolumn{1}{l|}{I was \#overloading my teammates}\\\hline
\multicolumn{2}{|c|}{\textbf{Example 4}}\\\hline
src&\<معينة>
traffic within period 
\<ال>
detect   
\<ن>\\
trg&\multicolumn{1}{l|}{to \#detect the \#traffic \#within a certain \#period}\\\hline
\end{tabular}
\caption{ArzEn Corpus Examples.}
\label{table:arzen_examples}
\end{table}
\end{comment}

%Slight modifications to English words are allowed for better fluency. For example:\\
%item Modifications to English words are allowed to handle morphological CS. For example:\\
%It is allowed to insert translations of neighboring Arabic words within a CS English segment for fluency

%%Given that Egyptian Arabic is a morphologically rich language \cite{HEH12}, Egyptians attach Arabic clitics and affixes to English words when code-switching. Morphological CS is present in Arzen, mostly occurring with clitics (88\%). Among the CS sentences, 45\% contain morphologically code-switched words. Morphological CS exacerbates the CS data sparsity problem, as it results in higher OOV rates. 

==> sections/intro_old.tex <==
\section{Introduction}
%%%Code-switching introduces a set of challenges to NLP systems. Data sparsity is one of the main bottlenecks hindering the development of CS NLP applications \cite{CV16}. Another int1eresting challenge is morphological CS. Besides CS occurring at the level of sentence boundaries (inter-sentential CS) and words (intra-sentential CS), CS also occurs at the level of morphemes (intra-word CS or morphological CS). This phenomenon occurs in the case of morphologically rich languages, where affixes in the primary language can get attached to words in the secondary language. 
Code-switching (CS) is the alternation of language in text or speech. CS can occur at the levels of sentences (inter-sentential CS), words (intra-sentential CS/code-mixing), and morphemes (intra-word CS or morphological CS). Data sparsity is one of the main bottlenecks hindering the development of CS NLP applications \cite{CV16}. 
\begin{comment}
Morphological CS occurs in the case of morphologically rich languages, where affixes in the primary language get attached to words in the secondary language. 
This directly affects the performance of machine translation (MT) systems. For example, the monolingual sentence (1) is correctly translated by Google Translate to `She concentrates on her work'. However, the equivalent CS sentence (2), which includes the prefix $^{\dagger}$\<بت>~{\it bit} `progressive-imperfect-3rd-fem-sing', is incorrectly translated to `She is a bit concentrate at her job'.\newline
\-\hspace{5mm}(1) \<هي بتركز في شغلها>\newline
\-\hspace{5mm}(2) \<في شغلها> concentrate $^{\dagger}$\<هي بت>
\end{comment}
Given that CS data is scare and that collecting such data is expensive and time-consuming, data augmentation serves as a solution that has proved to be successful at alleviating data sparsity. Most of the work done for CS data augmentation has been focused on language modeling, mostly for ASR rescoring. Several data augmentation techniques have been proposed based on linguistic theories \cite{PBC+18,LYL19}, heuristics \cite{SWY+11,VLW+12,KAT+21}, neural networks \cite{CCL18,WMW+18,WMW+19,LV20}, and machine translation \cite{TKJ21}. 

CS data augmentation has has been less investigated for the task of MT. The approaches mainly involved relying on parallel corpora and replacing source segments with their corresponding target segments. Replacements can be done using word alignments \cite{AGE+21,GVS21,XY21} or phrase tables \cite{MLJ+19,SZY+19}. 
%, or parse trees under the Equivalence Constraint . 
%In \cite{AGE+21}, all source words (except for stopwords) are replaced by the corresponding target words if one-to-one alignments exist. However, this will lead to over-modeling of CS as well as generation of CS sentences that are not linguistically correct. 
% if the order of words in not maintained across both languages.
Researchers have also applied linguistic constraints for data augmentation \cite{RSG+21,HCA+22}. In \cite{RSG+21}, the authors provide the GCM tool which utilizes the equivalence constraint \cite{Pop00} to generate CS sentences. However, linguistic theories are not guaranteed to provide generalization across languages, especially for languages with syntactic divergence, such as Arabic and English. By looking into the output of the GCM tool for the Arabic-English language pair, we notice that some sentences suffer from information loss, where the augmented sentences are incomplete, which was also reported in \cite{HCA+22}.

%In this paper, we investigate data augmentation for improved MT under the setting of a CS low-resource and morphologically rich language. We propose a novel method that combines Seq2seq model for predicting CS points with alignments of parallel corpora to create synthesized CS data. This language-agnostic approach achieves significant improvements in OOV rates and BLEU scores. By integrating morphological analysis, we tailor our system to handle morphological CS, achieving further gains. Finally, we show that appending target-target pairs to training data is a simple, yet effective, approach to tackle the problem of dropping foreign words in translation. Our best model achieves +8 BLEU points over the baseline model.
In this paper, we investigate lexical replacement for augmenting Arabic-English CS data. Specifically, we consider whether a neural-based predictive model can be trained to predict CS switch points. The training of the predictive model is done using limited amounts of CS data, and the model is then used to convert monolingual Arabic-English parallel data into CS-English data, by projecting the chosen words from the target to the source side. This has only been previously investigated for Hindi-English by \newcite{GVS21}. In this paper, we provide further experiments, exploring the use of different types of alignments. We evaluate the effectiveness of using the augmented data for LM, MT, and ASR rescoring tasks. We also evaluate the quality of the generated synthetic sentences through human evaluation. Through our study we aim at answering the following research questions: (RQ1) Can we utilize a trained sequence-to-sequence model that learns CS point prediction to produce synthetic CS data that mimics the CS style of natural CS data? (RQ2) Do improvements in synthetic data quality necessarily result in improvements in downstream tasks? For RQ1, based on our intrinsic evaluation and human evaluation, we observe that the approach relying on a trained predictive model to decide on CS points is able to mimic natural CS sentences to some extent and was found to be more acceptable by human annotators than synthetic data produced with random-based CS point predictions. For RQ2, we find that it partially holds in our case, where the use of a predictive model outperforms random-based CS point selections on all extrinsic tasks when 1-1 alignments are used, however, with the use of minimal unit alignments, where we perform segment replacements, the synthetic data produced by the random-based approach becomes more acceptable compared to using 1-1 alignments and are able to outperform using trained predictive models on extrinsic tasks.%provides augmentations that are less acceptable but possibly cover a wider range of CS styles.
%We also contribute with the collection and release of the first code-switched Arabic-English parallel corpus. The corpus includes the translation of ArzEn 12-h conversational speech corpus \cite{HVA20}, and thus involves natural code-switching. The corpus is a valuable resource that can be used for both data augmentation and machine translation tasks.

This paper is organized as follows. We present our ArzEn parallel corpus in Section \ref{sec:arzenMT}. In Section \ref{sec:data_augmentation}, we discuss the data augmentation approaches. We outline the experimental setup in Section \ref{sec:experimental_setup} and results in Section \ref{sec:results}. Finally, we provide further discussion in Section \ref{sec:discussion} and conclude in Section \ref{sec:conclusion}.

%leveraging parallel monolingual translations from a limited source of code-switching data.
%However, these constraints cannot be postulated as a universal rule for all code-switching scenarios, especially for languages that are syntactically divergent (Berk- Seligson, 1986), such as English and Mandarin since they have word alignments with an inverted order.
%Creating a large-scale code-switching dataset is also very expensive. Therefore, code-switching data generation methods to augment existing datasets are a useful workaround.

==> sections/linguisticAnalysis.tex <==
%\section{CS Eg-En Morphological Complexity}
%Eg-En CS Linguistic Analysis/
Egyptian Arabic, as Modern Standard Arabic, is a morphologically rich language \cite{HEH12}. 
\begin{comment}
\injy{@Prof. Nizar: I mimicked your example here, is that alright? Would you like us to write this section differently?}
For example, the word 
\<فحتلغيهاله> 
(fa+Ha+ti-log-iy+hA+l+uh) `so you will cancel it for him' includes 
two proclitics ( \<ف> fa+ 'so' and Ha+ `will'), 
one indirect pronominal object enclitic (\<له> +l+uh `for him'),  
one pronominal enclitic (\<ها> +hA `it'), 
and one circumfix (\<ت>+\<ي> ti- -iy+ 2rd person). 
%one prefix (ti+ 3rd person (fem.)), and one suffix (+iy )
%diac:حَتِلْغِي lex:لَغَى_1 bw:Ha/FUT_PART+ti/IV2FS+log/IV+iy/IVSUFF_SUBJ:2FS
%example: famanelgheehash/fahatelghehaloh
\end{comment}
When code-switching, Egyptians attach Arabic clitics and affixes to English words. 
%inject the same morphology into English words. 
%For example, the word `\<فحتلغيهاله>' becomes  
%`\<يهاله>
%cancel
%\<فحت>'.
In Table \ref{table:arzen_affixes}, we report the clitics and affixes present in ArzEn corpus along with their frequencies. We observe that morphological CS mostly involves the use of clitics (88\%) than affixes (12\%). %We observe that Egyptian Arabic clitics and affixes are mostly covered (need to check that) except for the circumfix negation \<ما>+ +\<ش> mA+ +\u{s} which is used to negate verbs. 
%The circumfix is also found within Egyptian-Arabic CS, for example \<ماتلغيهاش> (mA+ti-log-iy+hA+\u{s}) `don't cancel it' becomes 
%\<يهاش>
%cancel
%\<مات>. 
The morphological complexity of the Arabic language further adds to the problem of CS data sparsity, as different clitics and affixes can be attached to the embedded English words resulting in a large number of compound words, thus contributing to higher OOV rates. 

==> sections/rw_old.tex <==
\section{Related Work}
\begin{itemize}
    \item CS Data Augmentation
    \item CS MT
    \item (Arabic MT?)
\end{itemize}

\begin{comment}

\cite{AGE+21} utilize existing English-Hindi parallel data to generate code-mixed data. They first obtain alignments between source and target sentences, and replace the source token with the aligned target tokens. The authors treat all one-to-one alignments as candidates for replacement (except for stopwords), which can lead to over-modeling of CS, as well as generation of CS sentences that are not linguistically correct.

Similar to our approach, \cite{GVS21} rely on NN-based approach to learn CS points. As a first step, they use code-mixed sentence , label it with language IDs, and translate English words to their monolingual equivalents. They then train an m-BERT model on this sequence-labeling task, where the model learns to detect which words should be switched on the source monolingual side. Afterwards, replacements are done using word alignments. We did not opt for this approach, as our corpus is highly code-switched corpus, with English segments ranging from x-y consecutive English words, and therefore, translating whole segments word-by-word will not give a correct source monolingual sentences to train the model on. Instead, we opted to learn the CS points on the target side. Give an example of a sentence with influent translation. + order may change (possessive form).



As stated in \cite{CV16}, data scarcity is one of the main bottlenecks hindering the development of CS NLP systems.  

In the task of CS language modeling, some data augmentation techniques require one step such as using RNN for text generation. Most of the techniques however perform data generation on two steps; identifying the words in the primary language that should be replaced and identifying the alternative words in the secondary language. For the former task, researchers have first investigated the use of linguistic knowledge such as the Equivalence Constraint \cite{PBC+18}. Later on, with the advancements in neural networks, researchers have relied on NN for identifying CS words. For the latter task, researchers have relied on dictionaries, word embeddings, language models such as BERT, as well as parallel data.\\

\cite{VLW+12}: identified common CS embeddings and replaced their equivalent monolingual words with these segments, where replacements followed heuristics including trigger words and POS tags.

\cite{WN17}: relied on word embeddings

Generative adversarial neural network is also proposed to
learn code-switching point distribution from code-switching
text [12].

 The first work to study the use of linguistic theories for this purpose is by Li and Fung
[24], who used the assumption of the equivalence constraint [1, 24, 66] and functional head
constraint [67]. Instead of using linguistic theories, other studies have developed methods that
use a neural-based approach for data augmentation to learn the code-switching data distribution,
such as SeqGAN [68] and an encoder-decoder model with a copy mechanism [28].

%\cite{CCL18} proposed using GANs along with reinforcement learning to generate augmented sentences without the reliance on labeled data. The GAN learns to 

%In contrast to the task of data augmentation for language modeling, where a word in the primary language can be replaced by a similar word, replacements in data augmentation for machine translation are more restricted to either the actual word in the target text, or a synonym.


\end{comment}
